The distance to NGC1316 (Fornax A): yet another curious case

The distance of NGC1316, the brightest galaxy in Fornax, is an interesting test for the cosmological distance scale. First, because Fornax is the 2nd largest cluster of galaxies at <~25 Mpc after Virgo and, in contrast to Virgo, has a small line-of-sight depth; and second, because NGC1316 is the galaxy with the largest number of detected SNeIa, giving the opportunity to test the consistency of SNeIa distances internally and against other indicators. We measure SBF mags in NGC1316 from ground and space-based imaging data, providing a homogeneous set of measurements over a wide wavelength interval. The SBF, coupled with empirical and theoretical calibrations, are used to estimate the distance to the galaxy. We present the first B-band SBF measurements of NGC1316 and use them together with the optical and near-IR SBF data to analyze the properties of field stars. Our distance modulus m-M=31.59 +-0.05(stat) +-0.14(sys), when placed in a consistent Cepheid distance scale, agrees with the results from other indicators. However, our result is ~17% larger than the most recent estimate based on SNeIa. Possible explanations for this disagreement are the uncertainties on internal extinction, or calibration issues. Concerning the stellar population analysis, we confirm earlier results from other indicators: the field stars in NGC1316 are dominated by a solar metallicity, intermediate age component. A substantial mismatch exists between B-band SBF models and data, a behavior that can be accounted for by an enhanced percentage of hot horizontal branch stars. Our study of the SBF distance to NGC1316, and the comparison with distances from other indicators, raises some concern about the homogeneity between the calibrations of different indicators. If not properly placed in the same reference scale, significant differences can occur, with dramatic impact on the cosmological distance ladder.

==> tab_accuracy.tex <==
\begin{table}
\caption{Median $\bar{m}$ and $(\bar{m}{-}\bar{M})$ errors from the
literature}
\label{tab_accuracy}
\centering
\begin{tabular}{l c c l c }
\hline\hline 
Sample               & $\delta(\bar{m})$ & $\delta(\bar{m}{-}\bar{M})$  & Filter         & Number of sources  \\
                     &   (mag)           &       (mag)                  &                & (space/ground obs.) \\
\hline
\multicolumn{5}{c}{Optical bands} \\
\citet{tonry01}      &   0.18  &    0.20  &      $I$                  &      280 (ground)    \\
\citet{cantiello07b} &   0.02  &    0.09  & $F814W$($\sim I$)        &       13 (space) \\
\citet{blake09}      &   0.04  &    0.08  & $F850LP$($\sim g_{SDSS}$)  &      134 (space) \\
\citet{blake10b}     &   0.02  &    0.07  &  $F814W$($\sim I$)       &        9 (space) \\
\hline
\multicolumn{5}{c}{Near-IR bands} \\
\citet{jensen98}     &   0.14  &    0.19  & $K'$                    &       16   (ground)   \\
\citet{liu02}        &   0.07  &    0.20  & $K_S$                    &       19  (ground)   \\
\citet{jensen03}     &   0.08  &    0.17  & $F160W$ ($\sim H$)       &       79 (space) \\
\hline\hline 
\end{tabular} \\
\end{table}


==> tab_deltas.tex <==
\begin{table}
\caption{Nearby galaxy sample used for near--IR calibration: original and revised distances.}
\label{tab_deltas}
\centering
\begin{tabular}{l c l c c c}
\hline\hline 
Galaxy               & $\mM_{near-IR}$ &  Reference        & Method     & $\mM_{Revised}$&      $\Delta(Revised-Orig.)$ \\
\hline 
NGC\,4526            &  31.08    & \citet{krisciunas04a} & SBF        &    31.08    &       +0.00  \\
NGC\,4536            &  30.80    & \citet{krisciunas04a} & Cepheids   &    30.87    &       +0.07  \\
NGC\,3368            &  29.97    & \citet{krisciunas04a} & Cepheids   &    30.11    &       +0.14  \\
NGC\,4374            &  31.32    & \citet{krisciunas04b} & SBF        &    31.26    &       $-$0.06  \\
NGC\,3190(NGC\,3226) &  31.86    & \citet{krisciunas04b} & SBF        &    31.80    &       $-$0.06  \\
NGC\,936             &  31.65    & \citet{krisciunas09}  & SBF        &    31.75    &       +0.10  \\
NGC\,1201            &  31.37    & \citet{krisciunas09}  & SBF        &    31.47    &       +0.10  \\
NGC\,1371(Eridanus group) & 31.84& \citet{krisciunas09}  & SBF        &    31.94    &       +0.10  \\
NGC\,5128            &  27.90    & \citet{krisciunas09}  & SBF        &    28.06    &       +0.16  \\
\hline 
\multicolumn{5}{l}{Average (median) correction on the sample of nearby galaxies}    &  0.06$\pm$0.03 (0.085)            \\
\multicolumn{5}{l}{Average correction on the complete sample of galaxies (assume zero for distant galaxies)}  &  0.02$\pm$0.01          \\
\hline\hline 
\end{tabular} \\
\end{table}


==> tab_distances4.tex <==
\begin{table}
\caption{Distances from SBF  measurements.}
\label{tab_distances}
   \begin{center}
\begin{tabular}{l r c c}
\hline\hline 
Passband          & $\bar{M}$ calibration eq.                   &  $(m-M)$       & Reference        \\
\hline
\multicolumn{4}{c}{Empirical calibrations} \\
\hline 
$V$               & $(0.83\pm0.12)+(5.3\pm0.8)[(V{-}I)-1.15]$   & 31.53$\pm$0.17 &  [1]             \\ 
$I$               & $(-1.68\pm0.08)+(4.5\pm0.25)[(V{-}I)-1.15]$ & 31.65$\pm$0.12 &  [2]             \\ 
$I$               & $(-1.6\pm0.1)+(3.0\pm0.3)[(B{-}I)-2.0]$     & 31.55$\pm$0.13 &  [3]             \\ 
$z$  & $-$2.04+1.41$x$+2.60$x^2$+3.72$x^3$, $x\equiv(g{-}z)-1.94$& 31.66$\pm$0.07 & [4]  \\
$J_{F110W}$               & \nodata                                     & \nodata       & \nodata                      \\
$H_{F160W}$               & $(-4.8\pm0.1)+(5.1\pm0.5)[(V{-}I)-1.16]$    & 31.3$\pm$0.2  &   [5]        \\ 
$H_{F160W}$               & $-5.17+0.70x+2.90x^2$, $x\equiv(g{-}z)-1.94$      & 31.4$\pm$0.2   &   [6]        \\ 
\multicolumn{2}{r}{Weighted Mean}                               &31.59$\pm$0.05 &                              \\
\hline\hline 
\multicolumn{4}{c}{Theoretical calibrations} \\
\hline 
$V$ &   $0.89+4.01 [(V{-}I)-1.15]$  (0.3)                          & 31.4 $\pm$0.3   &                     \\
$I$ &  $-1.63+5.11 [(V{-}I)-1.15]$  (0.3)                          & 31.6 $\pm$0.3   &                     \\
$I$ &  $-1.63+2.65 [(B{-}I)-2.0] $  (0.3)                          & 31.6 $\pm$0.3   &                     \\
$z$ &  $-2.77+2.06 [(g{-}z)-1.94]$  (0.2)                         & 31.8 $\pm$0.2 &                     \\
$J_{F110W}$ &  $-3.75+3.07 [(V{-}I)-1.16]$  (0.3)                          & 31.3 $\pm$0.3   &                     \\
$H_{F160W}$ &  $-4.86+3.59 [(V{-}I)-1.16]$  (0.3)                          & 31.4 $\pm$0.4   &                     \\
\multicolumn{2}{r}{Weighted Mean}                                  & 31.60$\pm$0.11  &                        \\
\hline 
\end{tabular}
	\end{center}
\tablefoottext{1}{\citet{bva01}}\\ \tablefoottext{2}{\citet{tonry01}
  with revised Cepeheid
  distances}\\ \tablefoottext{3}{\citet{cantiello05}}\\ \tablefoottext{4}{Calibration
  using \citet{blake09}, uncertainties evaluated from eq. (1) in
  \citet{mei07xiii}}\\ \tablefoottext{5}{Calibration from
  \citet{jensen03} with metallicity correction on Cepheids and NICMOS to
  WFC3 $H_{F160W}$ zeropoint correction (see text).}\\ \tablefoottext{6}{Calibration from
  \citet{cho13}.}\\
\end{table}


==> tab_obs.tex <==
\begin{table}
\caption{Main properties of NGC\,1316.}
\centering
\begin{tabular}{l c}
\hline\hline
Alternative names                      &  Fornax A, FCC\,21, Arp\,154, ESO\,357-G\,022 \\
RA(J2000)$^{\mathrm{1}}$                   &   03h22m41.7s      \\
Dec(J2000)$^{\mathrm{1}}$                  &   $-$37d12m30s       \\
Galaxy Type$^{\mathrm{2}}$	                &   S0		     \\
Morphological Type$^{\mathrm{2}}$          &  $-$1.8$\pm$0.7	     \\
Absolute $B$-band magnitude$^{\mathrm{2}}$ &	$-$22.5 mag       \\
Recorded SNe Ia events	                       & SN1980N, SN1981D, SN2006dd, SN2006mr \\
$cz^{\mathrm{1}}$ (km/s, Heliocentric)    &  1788$\pm$10  	     \\
$E(B{-}V)^{\mathrm{3}}$                   &  0.021 mag    	     \\
$(V{-}I)_0^{\mathrm{4}}$		       & 1.132 $\pm$ 0.016 mag  \\
\hline
\end{tabular}
\begin{list}{}{}
\item[$^{\mathrm{1}}$] Data retrieved from NED (http://nedwww.ipac.caltech.edu); 
$^{\mathrm{2}}$  Hyperleda (http://leda.univ-lyon1.fr);
$^{\mathrm{3}}$ \citet{sfd98};
$^{\mathrm{4}}$  \citet{tonry01}
\end{list}
\label{tab_obs}
\end{table}


==> tab_qc_long.tex <==
\begin{center}
\tiny
\begin{longtable}{lllll}
\caption[Quality control statistics for the exposures.]{Quality control statistics for the exposures.} \label{QC} \\
\hline\hline	
	\noalign{\smallskip}
  File	Name & Background  & Background & seeing & Data Used \\ 
	-	& (counts) & ($mag/arcsec^2$) & ($\arcsec$) & - \\
	\hline
\multicolumn{5}{c}{$B$ band} \\
FORS.1999-12-28T02:42:27.813.fits & 888.0 & 22.25 & 0.86 & yes \\
FORS.1999-12-28T02:54:22.346.fits & 907.4 & 22.22 & 0.81 & yes \\
FORS.2000-01-09T02:41:46.659.fits & 983.8 & 22.13 & 1.07 & yes \\
FORS.2000-01-09T02:52:43.240.fits & 998.9 & 22.12 & 1.01 & yes \\
FORS.2000-01-12T01:11:59.202.fits & 1556.3 & 21.64 & 1.06 & yes \\
FORS.2000-01-12T01:22:57.678.fits & 1527.3 & 21.66 & 1.12 & yes \\
FORS.2000-01-13T00:56:41.525.fits & 2319.5 & 21.20 & 1.20 & yes \\
FORS.2000-01-13T01:07:40.539.fits & 2236.8 & 21.24 & 1.14 & yes \\
FORS.2000-01-14T03:50:58.405.fits & 1958.7 & 21.39 & 1.15 & yes \\
FORS.2000-01-14T04:01:58.759.fits & 1580.1 & 21.62 & 1.19 & yes \\
FORS.2000-01-15T03:10:31.420.fits & 7298.6 & 19.96 & 0.77 & no \\
FORS.2000-01-15T03:21:27.996.fits & 7231.2 & 19.97 & 0.86 & no \\
FORS.2000-01-17T03:28:21.613.fits & 11877.6 & 19.43 & 1.36 & no  \\
FORS.2000-01-17T03:39:19.186.fits & 12162.4 & 19.40 & 1.30 & no  \\
FORS.2000-01-18T01:20:21.447.fits & 12832.7 & 19.35 & 0.87 & no \\
FORS.2000-01-18T01:31:20.684.fits & 12983.9 & 19.33 & 0.77 & no  \\
FORS.2000-01-19T01:30:49.601.fits & 20047.5 & 18.86 & 1.38 & no  \\
FORS.2000-01-19T01:41:43.505.fits & 21026.0 & 18.81 & 1.31 & no  \\
FORS.2000-01-20T02:36:07.201.fits & 32829.0 & 18.33 & 1.15 & no  \\
FORS.2000-01-20T02:47:02.044.fits & 37640.4 & 18.18 & 0.70 & no  \\
FORS.2000-01-21T01:58:13.531.fits & 35260.4 & 18.25 & 0.70 & no  \\
FORS.2000-01-21T02:09:11.551.fits & 35681.1 & 18.24 & 0.70 & no  \\
	\hline
\multicolumn{5}{c}{$V$ band} \\
FORS.2000-01-09T03:28:34.384.fits & 3261.5 & 21.13 & 0.91  & yes\\
FORS.2000-01-09T03:39:32.352.fits & 3333.3 & 21.10 & 1.10 & yes \\
FORS.2000-01-13T01:20:04.617.fits & 10012.2 & 19.91 & 0.98 & yes \\
FORS.2000-01-13T01:31:04.242.fits & 69.2 & 19.93 & 0.84 & yes \\
FORS.2000-01-13T01:39:32.083.fits & 5141.9 & 20.63 & 1.03 & yes \\
FORS.2000-01-13T01:50:31.241.fits & 5130.5 & 20.64 & 1.09  & yes\\
FORS.2000-01-17T04:16:19.860.fits & 24234.6 & 18.95 & 1.51 & no \\
FORS.2000-01-17T04:27:17.584.fits & 25234.8 & 18.91 & 1.59 & no  \\
FORS.2000-01-18T02:06:59.548.fits & 25642.0 & 18.89 & 0.76 & no  \\
FORS.2000-01-18T02:17:56.431.fits & 23947.3 & 18.96 & 0.93 & no  \\
FORS.2000-01-19T01:07:22.117.fits & 38819.6 & 18.44 & 1.21 & no  \\
FORS.2000-01-19T01:18:19.487.fits & 37909.1 & 18.46 & 1.28 & no  \\
FORS.2000-01-20T01:52:46.180.fits & 22531.1 & 18.28 & 1.25 & no  \\
FORS.2000-01-20T01:58:44.418.fits & 29233.8 & 17.99 & 1.36 & no  \\
FORS.2000-01-20T02:05:45.069.fits & 39325.9 & 17.67 & 0.95 & no  \\
FORS.2000-01-20T02:11:42.821.fits & 38475.5 & 17.70 & 0.76 & no  \\
FORS.2000-01-21T00:54:09.577.fits & 6202.4 & 17.93 & 1.14 & no \\
FORS.2000-01-21T01:06:08.681.fits & 5118.1 & 18.14 & 1.06 & no  \\
FORS.2000-01-21T01:30:59.576.fits & 16978.9 & 18.14 & 1.09 & no  \\
FORS.2000-01-21T01:35:17.720.fits & 17047.7 & 18.14 & 1.11 & no  \\
FORS.2000-01-21T01:39:35.548.fits & 15737.2 & 18.23 & 0.98 & no  \\
FORS.2000-01-21T01:43:50.433.fits & 15366.4 & 18.25 & 1.03 & no  \\
FORS.2000-01-21T01:48:07.248.fits & 15653.2 & 18.23 & 1.06 & no  \\
FORS.2000-01-21T01:52:24.597.fits & 16583.5 & 18.17 & 1.08 & no  \\
            \hline
\multicolumn{5}{c}{$I$ band} \\
FORS.1999-12-27T03:46:00.987.fits & 9675.7 & 19.07 & 0.69 & yes \\
FORS.1999-12-27T03:57:55.778.fits & 10469.2 & 18.99 & 0.78 & yes \\
FORS.2000-01-09T03:05:09.924.fits & 8138.7 & 19.26 & 0.87 & yes \\
FORS.2000-01-09T03:16:07.432.fits & 8755.6 & 19.18 & 0.82 & yes \\
FORS.2000-01-13T02:03:14.285.fits & 9061.0 & 19.14 & 0.93 & yes \\
FORS.2000-01-13T02:14:12.265.fits & 9847.6 & 19.05 & 0.84 & yes \\
FORS.2000-01-15T03:34:22.320.fits & 19878.0 & 18.29 & 0.79 & yes \\
FORS.2000-01-15T03:45:21.020.fits & 20169.8 & 18.27 & 1.00 & yes \\
FORS.2000-01-17T03:52:07.180.fits & 18776.9 & 18.35 & 1.22 & no \\
FORS.2000-01-17T04:03:05.404.fits & 19359.7 & 18.32 & 1.36 & no  \\
FORS.2000-01-18T01:43:30.890.fits & 19114.6 & 18.33 & 0.65 & no  \\
FORS.2000-01-18T01:54:29.531.fits & 19684.5 & 18.30 & 0.74 & no  \\
FORS.2000-01-19T00:44:09.869.fits & 27488.0 & 17.94 & 1.13 & no  \\
FORS.2000-01-19T00:55:07.408.fits & 28624.7 & 17.89 & 1.09 & no  \\
FORS.2000-01-21T02:22:08.776.fits & 16986.9 & 17.71 & 1.01 & no  \\
FORS.2000-01-21T02:28:02.578.fits & 17131.9 & 17.70 & 1.05  & no \\
FORS.2000-01-21T02:33:59.741.fits & 16976.3 & 17.71 & 0.99  & no \\
FORS.2000-01-21T02:39:57.532.fits & 16960.7 & 17.71 & 1.08  & no \\
FORS.2000-02-04T02:06:34.213.fits & 9268.9 & 19.12 & 1.03 & yes \\
FORS.2000-02-04T02:17:28.971.fits & 8959.7 & 19.16 & 0.85 & yes  \\

             \noalign{\smallskip}
            \hline\\
      
\end{longtable}
\end{center}


==> tab_sbf2.tex <==
\begin{table}
\caption{Surface Brightness Fluctuations and colors measurements corrected for galactic extinction.}
\label{tab_sbf}
\centering
\begin{tabular}{c c c c c c}
\hline\hline 
\multicolumn{6}{c}{VLT data} \\
\hline 
$\langle r \rangle$ &  $B{-}V$ & $V{-}I$ &  $\bar{B}$ &  $\bar{V}$ &$\bar{I}$  \\
    (arcsec)        &    (mag) &   (mag)  & (mag)     &  (mag)     &  (mag)    \\
 170    &   0.84 $\pm$0.03 &   1.116 $\pm$0.015 &  33.02 $\pm$0.02 &  32.19 $\pm$0.09 &  29.81 $\pm$0.07  \\
\hline
\multicolumn{3}{c}{PSF uncertainty} & 0.09 & 0.04 & 0.03 \\
\hline\hline 
\multicolumn{6}{c}{ACS data} \\
\hline 
 $\langle r \rangle$ &  $g{-}z$ &         &  &          &   $\bar{z}$       \\
     (arcsec)        &    (mag) &         &  &          & (mag)             \\
 80                  &  1.954 $\pm$0.011 &     &  &          & 29.11$\pm$  0.06        \\
\hline 
\multicolumn{3}{c}{PSF uncertainty} &    &  & 0.014 \\
\hline\hline 
\multicolumn{6}{c}{WFC3/IR data} \\
\hline 
$\langle r \rangle$ &  $V{-}I$$^{\mathrm{a}}$ & $J{-}H$        &  &   $\bar{J}$       &   $\bar{H}$       \\
    (arcsec)        &    (mag) &                &  &   (mag)           & (mag)             \\
 80  & 1.102 $\pm$0.002 & 0.72 $\pm$0.01 & &   27.32$\pm$ 0.07&   26.28 $\pm$0.04  \\
\hline 
\multicolumn{3}{c}{PSF uncertainty} &    &  0.2 & 0.2 \\
\hline\hline 
\end{tabular}
\begin{list}{}{}
\item
[[$^{\mathrm{a}}$]] Colour data obtained from VLT data using the same
masks adopted for WFC3/IR measurements.
\end{list}
\end{table}


==> tab_sbfpnlf2.tex <==
\begin{table}
\caption{SBF to PNLF comparison.}
\label{tab_sbfpnlf}
\centering
\begin{tabular}{l c c c}
\hline\hline 
Sample                       & Number of galaxies &  $\Delta_{PNLF-SBF}$ ($rms$) &  Median difference  \\
                             &                    &      (mag)          &            (mag)    \\
\hline
Original$^\mathrm{[1]}$        &        28          &   $-$0.36  (0.31)  &    $-$0.36            \\   
a$^\mathrm{[2]}$               &        28          &   $-$0.23  (0.31)  &    $-$0.23            \\
b$^\mathrm{[3]}$               &        33          &   $-$0.21  (0.29)  &    $-$0.23            \\
c$^\mathrm{[4]}$               &        33          &   $-$0.22  (0.30)  &    $-$0.29            \\
d$^\mathrm{[5]}$               &        33          &   $-$0.18  (0.34)  &    $-$0.26            \\
\hline
\end{tabular}
\begin{list}{}{}
\item [[1]] Original PNLF sample by \citet{ciardullo02} with SBF distances from \citet{tonry01}.
\item [[2]] \citet{tonry01} SBF \& \citet{ciardullo02} PNLF with revised zero points based on metallicity dependent PL relations for Cepheids (see text).
\item [[3]] \citet{tonry01} SBF \& \citet{ciardullo02} PNLF plus more
  recent PNLF distances from \citet[][NGC\,1380, NGC\,4526 and revised
    NGC\,1316]{feldmeier07}, \citet[][NGC\,4697]{sambhus06},
  \citet[][NGC\,1344 and NGC\,821,
    respectively]{teodorescu05,teodorescu10} and
  \citet[][NGC\,4376]{herrmann08}. For both distance indicators
  revised zero points are used, as in sample $b$ except for NGC\,4697, NGC\,1344 and
  NGC\,821 whose PNLF distance is independent from
  \citeauthor{ciardullo02} calibration.
\item [[4]] Updated SBF distances from ACSVCS \citep{cote04} \& ACSFCS
  \citep{jordan07} (when available).  Old SBF and PNLF distances as in
  sample $b$.
\item [[5]] As sample $c$ except that SBF with Q--corrected SBF
  distances (see text) are used for the old \citet{tonry01} distance
  moduli.
\end{list}
\end{table}


==> tab_sne2.tex <==
\begin{table}
\caption{Type Ia Supernova distances to NGC\,1316 available in the literature.}
\label{tab_sne}
\centering
\begin{tabular}{l c c c}
\hline\hline 
SN      & $\mM$            & Method   &  References/Notes         \\
\hline 
\multicolumn{4}{c}{Measurements from Str10} \\
80N+81D+06dd & 31.180 $\pm$ 0.013 & SNooPy EBV & Author's best estimate           \\
80N+81D+06dd & 31.25 $\pm$ 0.03 & Tripp      & Author's best estimate              \\
80N+81D+06dd & 31.203 $\pm$ 0.012 & $(m-M)_{max}$ Near-IR   & Author's best estimate         \\
SN\,2006mr     & 31.83 $\pm$ 0.07   & Tripp    & Flagged as doubtful        \\
SN\,2006mr     & 31.739 $\pm$ 0.005 &$(m-M)_{max}$ Near-IR    &     Flagged as doubtful     \\
\hline\hline 
\multicolumn{4}{c}{Other Measurements$^{\mathrm{a}}$} \\
SN\,1980N & 31.45             & $M_{max}$& \citet{hamuy91}\\
SN\,1981D & 31.35             & $M_{max}$& \citet{hamuy91}\\
\hline 
SN\,1980N & 31.44 $\pm$0.32   & MLCS     & \citet{krisciunas00}\\
SN\,1981D & 31.03 $\pm$0.3    & MLCS     & \citet{krisciunas00}\\
\hline 
SN\,1980N & 31.30 $\pm$0.15 & MLCS  & \citet{ajhar01}      \\
SN\,1980N & 31.51 $\pm$0.10 & $\Delta m_{15}$  & \citet{ajhar01}      \\
\hline 
SN\,1980N & 31.35             & $M_{max}$& \citet{reindl05}\\
SN\,1981D & 30.98             & $M_{max}$& \citet{reindl05}\\
\hline 
SN\,1980N & 31.38 $\pm$0.13 & MLCS2k2  & \citet{jha07}      \\
SN\,1981D & 30.78 $\pm$0.24 & MLCS2k2  & \citet{jha07}      \\
\hline 
SN\,2006dd & 31.34 $\pm$0.11 & MLCS   & \citet{maoz08}      \\
\hline\hline 
\end{tabular} \\
\tablefoottext{a}{All distances  are converted to a scale with
  $H_0=72~km~s^{-1}~Mpc^{-1}$.}
\end{table}


==> tab_times.tex <==
%__________________________________________________ One column table
   \begin{table}
   \begin{center}
      \caption[]{Total and used exposure times for each band.}
         \label{ObsLog}
         \begin{tabular}{lccc}
            \hline\hline
            \noalign{\smallskip}
          &  B (s) & V (s) &  I (s)\\
            \hline 
            \noalign{\smallskip}
            \noalign{\smallskip}
        Total available &  13200 & 9000  & 10800  \\
        Used  &    6000 & 3600  & 6000   \\
             \noalign{\smallskip}
            \hline
	\end{tabular}
	\end{center}
   
   \end{table}
%

